Maximizing Social Welfare in a Competitive Diffusion Model

Influence maximization (IM) has garnered a lot of attention in the literature owing to applications such as viral marketing and infection containment. It aims to select a small number of seed users to adopt an item such that adoption propagates to a large number of users in the network. Competitive IM focuses on the propagation of competing items in the network. Existing works on competitive IM have several limitations. (1) They fail to incorporate economic incentives in users' decision making in item adoptions. (2) Majority of the works aim to maximize the adoption of one particular item, and ignore the collective role that different items play. (3) They focus mostly on one aspect of competition -- pure competition. To address these concerns we study competitive IM under a utility-driven propagation model called UIC, and study social welfare maximization. The problem in general is not only NP-hard but also NP-hard to approximate within any constant factor. We, therefore, devise instant dependent efficient approximation algorithms for the general case as well as a $(1-1/e-\epsilon)$-approximation algorithm for a restricted setting. Our algorithms outperform different baselines on competitive IM, both in terms of solution quality and running time on large real networks under both synthetic and real utility configurations.

==> sec-algosdiscuss.tex <==
\subsection{ $\PRIMAP$ algorithm}
In this section we present the $\PRIMAP$ algorithm that \sgrd and \mgrd use to select the seed nodes. Before that we present the prefix preserving on marginal property formally.

\begin{definition}{\sc (Prefix-Preserving on Marginal Property).\ } \label{def:PRIMM}
	\fixedspaceword[.75]{Given $G$ $=$ $(V,E,p)$, budget vector $\bvec$ and a fixed seed set $S^P$, an influence maximization algorithm $\mathbb{A}$
	is prefix-preserving on marginal w.r.t. $\bvec$ and $S^P$, 
	if for any $\epsilon$ $>$ $0$ and $\ell$ $>$ $0$, 
	$\mathbb{A}$  returns an ordered set $\greedSeeds_{\bmax}$ of size $\bmax = \sum_{b_i \in \bvec} b_i$, 
	such that  with probability  at least $1$ $-$ $\frac{1}{|V|^{\ell}}$, 
	for every $b_i$ $\in$ $\bvec$, the top-$b_i$ nodes of $\greedSeeds_{\bmax}$, denoted $\greedSeeds_{b_i}$, satisfies $\sigma(\greedSeeds_{b_i} \mid S^P)$ $\geq$ $(1-\frac{1}{e} - \epsilon)$ $\OPT_{b_i \mid S^P} $, %\sigma(\optSeeds_{b_i})$, 
	where %$\optSeeds_{b_i}$ is the optimal seed set with $b_i$ seeds in the IC model.
	$\OPT_{b_i \mid S^P}$ is the optimal marginal expected spread of $b_i$ nodes on top the existing seeds $S^P$.}
\end{definition}


\begin{algorithm}[t!]

\caption{$\PRIMAP(G, \epsilon, \ell, S^P, \bvec)$} \label{alg:primap}
\begin{algorithmic}[1]
\State Initialize $\mathcal{R} = \emptyset$, $s = 1$, $n = |V|$, $i = 1$, $\epsilon^\prime = \sqrt{2} \cdot \epsilon$, $\budgetSwitch = \false$; 
\State $\ell = \ell  + \log 2 / \log n $, $\ell^\prime = \log_n(n^{\ell} \cdot |\bvec|)$;  \label{lin:ellb}
\While{$i \leq \log_2(n) - 1$ and $s \leq |\bvec|$} 
	\State $k = b_s$, $LB =1$; 
	\State $x = \frac{n}{2^i}$; $\theta_i = \lambda^\prime_k/x$, where $\lambda^\prime_k$ is defined in Eq. \eqref{eq:lambdap} \label{lin:lambdap} 
	\While{$|\mathcal{R}| \leq \theta_i$}                                   \label{lin:genr1}
		\State Generate an RR set $R$ for a randomly selected node $v$ of $G$
		 \State If $R$ does not contain any node of $S^P$, insert $R$ in $\mathcal{R}$; \label{lin:genr2}
	\EndWhile
	\If{$\budgetSwitch$}
		\State $S_k = $ the first $k$ nodes in the ordered set $S_{b_{s-1}}$ returned from
		the previous call to $\nodeselect$
	\Else 
		\State $S_k =\nodeselect(\mathcal{R}, k)$
	\EndIf
	\If{$n \cdot F_{\mathcal{R}}(S_k) \geq (1 + \epsilon^\prime)\cdot x$}  \label{lin:cov}
		\State $LB = n \cdot F_{\mathcal{R}(S_k)} / (1+\epsilon^\prime) $ 
		\State $\theta_k = \lambda^\ast_k / LB$, where $\lambda^\ast_k$ is defined in Eq. \eqref{eq:lambdaa} \label{lin:suc1}
		\While{$|\mathcal{R}|<\theta_k$} 
			\State Generate an RR $R$ set for a randomly selected node $v$ of $G$
			\State If $R$ does not contain any node of $S^P$, insert $R$ in $\mathcal{R}$    \label{lin:suc2}
		\EndWhile
		\State $s = s + 1 $; $\budgetSwitch = \true$	
	
	\Else 
		\State $i= i+1$; $\budgetSwitch = \false$
	\EndIf
	
\EndWhile
\If{$s \leq |\bvec|$}
	\State $\theta_k = \lambda^\ast_{b_s}/LB$ \label{lin:final}	
\EndIf	
\State $\mathcal{R} = \emptyset$
\While{$|\mathcal{R}|<\theta_k$}    \label{lin:weinote}
		\State Generate an RR $R$ set for a randomly selected node $v$ of $G$
			\State If $R$ does not contain any node of $S^P$, insert $R$ in $\mathcal{R}$
\EndWhile
\State $S_{\bmax} = \nodeselect(\mathcal{R}, \bmax)$ \label{lin:nodes}
\State \textbf{return} $S_{\bmax}$ as the final seed set
\end{algorithmic}
\end{algorithm}

We now present the $\PRIMAP$ algorithm that have the prefix preserving on marginal property. Pseudo code of $\PRIMAP$ is shown in Algorithm \ref{alg:primap}. 
In \cite{ban2019} authors proposed a prefix preserving IMM algorithm $\PRIMM$. For the given budget vector $\bvec$, $\PRIMM$ generates enough RR sets so that for any budget $k \in \bvec$, $|\mathcal{R}|\geq \lambda^\ast_k / \OPT_k$, with probability at least $1 - 1/n^{\ell^\prime}$. $\lambda^\ast_k$ and $\lambda'$ of Line \ref{lin:lambdap} is defined as follows,
\begin{equation}\label{eq:lambdap}
\lambda^\prime_k = \frac{(2+\frac{2}{3}\epsilon^\prime) \cdot (\log {n \choose k} + \ell^\prime \cdot \log \ n+\log\log_{2} \ n )\cdot n}{\epsilon^{\prime 2}},
\end{equation} 
\vspace*{-2mm}
\begin{gather}\label{eq:lambdaa}
\lambda^\ast_k = 2n \cdot ((1 - 1/e)\cdot \alpha + \beta_k)^2 \cdot \epsilon^{-2}, 
\end{gather} 
where, $\alpha = \sqrt{\ell' \log n + \log 2}$ is a constant independent of $k$, and 
$\beta_k = \sqrt{(1 - 1/e) \cdot (\log \tbinom{n}{k}+\ell^\prime \log \ n+ \log 2)}$.
Further since $OPT_k$ is unknown, $\PRIMM$ derives lower bounds $LB_k$ by iterating over $\bvec$ to find $|\mathcal{R}| = max_{k \in \bvec}\lambda^\ast_k/LB_k$. Finally the using $\mathcal{R}$, the seed nodes are selected 
solving the coverage problem greedily using $\nodeselect(\mathcal{R},k)$ \cite{tang15}. We extend $\PRIMM$ for the marginal case.

The difference between $\PRIMM$ and $\PRIMAP$ lies in type of RR set they use. While $\PRIMM$ includes RR set starting from any random node of $G$, $\PRIMAP$ includes only those RR sets that are not covered by the nodes of the existing seed set $S^P$. Therefore the approximation guarantee of $\PRIMAP$ holds on the graph that is not reached by the existing allocation. 

Correctness of $\PRIMAP$ follows from the proof of $\PRIMM$ \cite{ban2019}. In short, by selecting seeds from the uncovered portion of the graph, $\PRIMAP$ achieves the prefix preserving on marginal property. Theorem \ref{thm:main} follows from Lemmas \ref{lem:sgrd_bound}, \ref{lem:mgrd_bound}, \ref{lem:supgrd_bound} and the correctness of $\PRIMAP$.

\spara{Running time}

The running time of $\PRIMAP$ also follows the similar analysis of \cite{ban2019}. From Lemma $9$ of \cite{tang15}, we have for any budget $k$, the set of RR sets generated for that budget $\mathcal{R}_k$ satisfies, 

\begin{align*}
\mathbb{E}[|\mathcal{R}_k|] &\leq \frac{3 max\{ \lambda^\ast_k, \lambda^\prime_k\} \cdot (1+\epsilon^\prime)^2}{(1 - 1/e)\cdot \OPT_k}.
\end{align*}

Different from \cite{ban2019}, $OPT_k$ here is the marginal spread, instead of the absolute spread.
Since $\lambda^\prime_k$ and $\lambda^\ast_k$ are both monotone in $k$ (Eq. (\eqref{eq:lambdap}) and (\eqref{eq:lambdaa})), we know their maximums are achieved for $k = \bmax$, where $\bmax$ is the maximum budget in the budget vector. 
 
Further let $\OPT_{min} := \OPT_{b_{|{\bf I}|}}$ be the minimum possible value of the optimal expected marginal spread for any budget in the budget vector, then for any $\mathcal{R}_k$,
\begin{align*}
\mathbb{E}[|\mathcal{R}_k|] &\leq \frac{3 max\{ \lambda^\ast_{\bmax}, \lambda^\prime_{\bmax}\} \cdot (1+\epsilon^\prime)^2}{(1 - 1/e)\cdot \OPT_{min}} \\
& = O((\bmax+\ell^\prime)n\log \ n \cdot \epsilon^{-2} / \OPT_{min}).
\end{align*}

Further since $\PRIMAP$ reuses the RR sets instead of generating them from scratch for every budget, for the RR set $\mathcal{R}$ generated by $\PRIMAP$,

\begin{align}\label{eq:rsize}
\mathbb{E}[|\mathcal{R}|] &= max_{k \in \bvec}\{ \mathbb{E}[|\mathcal{R}_k|] \} \nonumber \\ 
& = O((\bmax+\ell^\prime)n\log \ n \cdot \epsilon^{-2} / \OPT_{min}).
\end{align}

For an RR set $R \in \mathcal{R}$, let $w(R)$ denote the number of edges in $G$ pointing to nodes in $R$. If $EPT$ is the expected value of $w(R)$. Since we build RR set only using uncovered nodes, $n \cdot EPT \leq m \cdot \OPT_{min}$ \cite{tang15}. Hence using Eq.~\eqref{eq:rsize}, the expected total time to generate $\mathcal{R}$ is determined by,
\begin{align}\label{eq:rtime}
\mathbb{E}[\sum_{R \in \mathcal{R}}w(R)] &= \mathbb{E}[|\mathcal{R}|] \cdot EPT \nonumber \\
& = O((\bmax+\ell^\prime)(n+m)\log \ n \cdot \epsilon^{-2}).
\end{align}
Since $\nodeselect$ involves one pass over all RR set, on a given input $\mathcal{R}_i$, it takes $O(\sum_{R \in \mathcal{R}_i} |R|)$ time. Recall $|\mathcal{R}_i|$ doubles with every increment of $i$. Hence it is a geometric sequence with a common ratio of $2$. Thus $\ell' = \ell + \log_n |\bvec|$. Hence the overall running time of $\PRIMAP$ is,
$$O((\bmax+\ell + \log_n |\bvec|)(n+m)\log \ n \cdot \epsilon^{-2})$$.
